Investigating and Recommending Co-Changed Entities for JavaScript Programs

JavaScript (JS) is one of the most popular programming languages due to its flexibility and versatility, but maintaining JS code is tedious and error-prone. In our research, we conducted an empirical study to characterize the relationship between co-changed software entities (e.g., functions and variables), and built a machine learning (ML)-based approach to recommend additional entity to edit given developers' code changes. Specifically, we first crawled 14,747 commits in 10 open-source projects; for each commit, we created one or more change dependency graphs (CDGs) to model the referencer-referencee relationship between co-changed entities. Next, we extracted the common subgraphs between CDGs to locate recurring co-change patterns between entities. Finally, based on those patterns, we extracted code features from co-changed entities and trained an ML model that recommends entities-to-change given a program commit. According to our empirical investigation, (1) three recurring patterns commonly exist in all projects; (2) 80%--90% of co-changed function pairs either invoke the same function(s), access the same variable(s), or contain similar statement(s); (3) our ML-based approach CoRec recommended entity changes with high accuracy (73%--78%). CoRec complements prior work because it suggests changes based on program syntax, textual similarity, as well as software history; it achieved higher accuracy than two existing tools in our evaluation.

==> methodology.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Methodology}
\label{sec:methodology}
This section first explains how we extracted recurring change patterns from CDGs across commits (Section~\ref{sec:rcp}), it then describes in detail how we built tools to create CDGs (Section~\ref{sec:changedistiller}, ~\ref{sec:binding}), Section~\ref{sec:suggester} illustrates how we designed \tool to suggest function co-changes for the top three patterns. We then presents the attribute set (Section~\ref{sec:attributes}) and machine-learning models (Section~\ref{sec:models}) used by \tool.
\subsection{Recurring change pattern Extraction}
\label{sec:rcp}
To investigate what kind of changes are co-applied and how changed entities are usually related, we first constructed CDG(s) for each given bug fix by extracting the changed entities and connecting them based on their syntactic dependence relations. The recurring change patterns were then identified by finding the largest common subgraph between CDGs.

\textbf{Step1: Extracting Changed Entities.}
We collect project history commits (old and new versions of JavaScript files) related to bug fix by using JGit\cite{jgit}, a Git client for Java. We identify bug-fix commits by detecting the commit message with matching key words such as "bug", "fix", "error", "adjust" and "failure". JavaScript Abstract Syntax Trees (ASTs) are generated and explored using ESprima\cite{esprima} and Typed-AST\cite{typed-ast}. Esprima is a high performance, standard-compliant JavaScript parser with full support for ECMAScript 2016 (ES6). Typed-AST is a tool developed by r2c for ASTs annotated with structured representations of TypeScript types. Both tools create ASTs in similar JSON format, however Typed-AST can provide additional inferred type information while ESprima can provide the whole token list. We used the hybrid of the two parsers to analyze the chosen JavaScript projects, except Node.js, since Typed-AST relies on "package.json" file to generate inferred type, whereas Node.js is a JavaScript runtime environment framework without dependencies on npm. 

AST differencing is performed using GumTreeDiff\cite{gumtree}, a fine-grained AST differencing tool which transforms JSON-format ASTs to gumTrees and computes differences between them. Though GumTreeDiff directly supports JavaScript source code differencing by applying Mozilla Rhino\cite{rhino} to generate ASTs, we do not use this functionality because Rhino doesn't support most syntax (e.g., imports, exports) in ES6\cite{rhinosupport}. One drawback of GumTreeDiff is that the generated gumTrees are too large and too complicated to deal with. The size of an AST JSON file is about 30 times larger than the size of the original JavaScript file, making the comparison between two entire JSON-format ASTs extremely time-costing. To handle this, we designed an entity extractor tool to first identify all the entities (classes, variables, functions, and expressions) from a JavaScript file, and then applly GumTreeDiff to compute the differences between matched entities. Our research leverages only those reported entity-level changes. 


\textbf{Step 2: Correlating Changed Entities.}
To determine if two changed entities ($E_1$ and $E_2$) are syntactically dependent, we check whether there is any access, containment or inheritance relationship between the entities. Then CDGs are constructed accordingly.
\begin{itemize}
  \item \textbf{Access} checks for any variable, function reference by an edited function or expression. If $E_1$'s implementation refers to $E_2$, we conclude that $E_1$ accesses $E_2$. 
  \item \textbf{Containment} checks for any overlap between code regions. If $E_1$'s code region is fully covered by $E_2$'s region, we conclude that $E_1$ is contained by $E_2$.
  \item \textbf{Inheritance} checks for class inheritance. If a class or objected function $E_1$ inherits (extends) another class or objected function $E_2$, we conclude that $E_1$ inherits $E_2$. 
\end{itemize}

\textbf{Step 3: Recurring change pattern identification}
We extracted recurring change patterns across the CDGs of different commits. Given two commits' CDGs: $GS_1 = \{cdg_{11},...,cdg_{1m}\}$ and $GS_2 = \{cdg_{21},...,cdg_{2n}\}$, we compared every pair of CDGs across commits (e.g., $< cdg_{11}, cdg_{21} >$) in an enumerative way. The comparsion of each pair starts with matching individual nodes based on their changed entity labels (e.g. \textbf{CF}), and proceeds with edge matching. If two edges (e.g., $e_1$ and $e_2$) have identical source changes, target changes, and edge directions, we consider them as matched. 

Based on such node and edge matches, we extracted the largest common subgraph between two CDGs with an off-the-shelf subgraph isomorphism algorithm VF2~\cite{Cordella2004:VF2}. Our implementation used JGraphT~\cite{jgrapht}, a Java graph library with a built-in implementation of VF2. Intuitively, VF2 treats the known node matches as initially identified common subgraphs. It then iteratively expands the subgraphs by incrementally adding more node and edge matches that do not conflict with the existing match(es). This process continues until no extra match can be added. When VF2 recognized multiple common subgraphs, we recorded the one covering the largest number of nodes, considering it as a recurring change pattern.

\subsection{Design of Change Distiller}
\label{sec:changedistiller}
As discussed in Section~\ref{sec:rcp}, since the AST JSON files are too large to handle by using GumTreeDiff, we extended GumTreeDiff by an Entity Extractor tool and a Change Distiller tool. We designed Entity Extractor to extract all the functions, classes, variables and expressions with their unique signatures from old and new versions of JavaScript files, we briefly talked about what these four kinds of entities represent in Section~\ref{sec:concepts}, here we describe them more concretely.
\begin{itemize}
    \item \textbf{A function} represents a method defined (1) directly in a JavaScript file (\codefont{function foo(...), var foo = function(...), exports.foo = function(...)}, etc.) with signature \codefont{pathToJsFile}-\codefont{.foo}; (2) inside an ES6 class  (\codefont{Class A \{ foo : function(...)\}}, etc.) with signature \codefont{pathToJsFile.A.foo}; (3) to extend the prototype of an objected function (\codefont{A.prototype.foo = function(...), \textunderscore.extend(A, \{foo : function(...)\})}, etc.) with signature \codefont{pathTo}-\codefont{JsFile.A.foo}; (4) in a CallExpression that returns a function, for example, \codefont{var foo = \textunderscore.once(function(...))}, where lodash \codefont{\textunderscore.once} method works by returning a function that will call the given function only once when called. 
    
    \item \textbf{A class} represents either an ES6 class or an ES5 objected function. In ES6, class A is defined as \codefont{Class A \{...\}}, inside which a constructor and several other methods are defined. The constructor of class A is treated as a function with signature \codefont{pathToJsFile.A.A}. In ES5, a function can be objected by using keyword "prototype" or by using lodash or underscore \codefont{\textunderscore.extend} method, and we call such function a class. For example, function A has been declared, then it is objected by \codefont{A.prototype = \{...\}} or \codefont{\textunderscore.extend(A, \{...\})}. In this case, we assign class A with signature \codefont{pathToJsFile.A}, whereas the function A is considered to be the constructor of class A, with signature \codefont{pathToJsFile.A.A}.   
    \item \textbf{A variable} represents a field declared directly in a JavaScript file (\codefont{var bar = ...}, etc) with signature \codefont{pathToJsFile.bar} or in a class constructor. In the constructor of class A, variables should be declared as \codefont{this.bar = ...} or \codefont{self.bar = ...} with signature \codefont{pathToJsFile.A.bar}. Statements like \codefont{var bar = ...} in a constructor are treated as declaration statements instead of variables. As we discussed in Section~\ref{sec:concepts}, an exception of variables is module require (Node.js) or module import (ES6), for instance in variable declaration \codefont{const config = require('/path/to/file')}, \codefont{config} represents a required module or an entity in file \codefont{'/path/to/file'}, one can simply ignore them when extracting program entities from JavaScript files.
    \item \textbf{An expression} represents a block of statements that doesn't belong to any function, class or variable. For instance, in most JavaScript files for testing, \codefont{describe()} method is often called separately to form a CallExpression. Other expressions can be IfStatement, WhileStatement, etc.. Since there is no initialization process for an expression, we do not give an expression a signature, that is to say, an expression can not be accessed by any entity. However to locate an expression we name it by using \codefont{pathToJsFile.positionOfExpression}.
\end{itemize}

We identify changed entities from the old and new versions of JavaScript files based on the extracted entity sets. For functions, classes and variables, since they have unique signatures, added entities (AF, AC, and AV) refer to those whose signatures only exist in the new version, deleted entities (DF, DC, and DV) refer to those whose signatures only exist in the old version, changed entities (CF, CV) refer to those whose signatures exist in both old and new versions, but with different gumTree shape (detected by gumTreeDiff with diff actions, since the size of an entity is much smaller than the whole JavaScript file, it is tolerable). If a function only changes its name in the new version, then the Change Distiller treats it as a deleted function and an added function since there are no matching function signatures between the old and new versions. For expressions, since they don't have signatures, we compare their token sequences. If the longest common subsequence between two expressions accounts for above 50\% of their average token sequence size, then we say those two expressions are matched and we extract a changed expression (CE) if they are not identical. From those expressions without matching to any other expressions, we extract deleted expressions (DE) in old versions and added expressions (AE) in new versions. 
\subsection{Design of Type Binding}
\label{sec:binding}
We connect changed entities by using the hybrid of our signature system and Typed-AST tool. The signature of an entity is in the format of \codefont{pathToJsFile.entityName}, where \codefont{pathToJsFile} is generated when mining bug fixes from github commits.

When TypedAST isn't applicable due to the lack of "package.json" file (project "Node.js"), the signature system is the only method to resolve bindings and connections with the usage of Esprima. In this case, to check whether $E_1$ accesses $E_2$, our tool traverse the Esprima AST body of $E_1$ to find whether there is a signature matching to $E_2$. For example, if $E_2$ is a function, all the "CallExpressions" in the body of $E_1$ AST are collected. If any callee function matches the signature of $E_2$, then we say $E_1$ accesses $E_2$. For $E_1$ and $E_2$ in different JavaScript files, we look up all the "require" and "import" statement locally in $E_1$ and globally in upper level of $E_1$ (the JavaScript file where $E_1$ is declared) to search for the imported module (JavaScript files) that contains $E_2$. However, without the support of Typed-AST, some entity identifications and some connections can be missing. For instance, let's say the right side of an "AssignmentExpression" contains a "CallExpression" which returns another function, \codefont{foo = bar(...)} where \codefont{bar(...)} returns a function, then this statement should be considered as a function declaration, and \codefont{foo} is a function instead of a variable or an expression. However, without the support of Typed-AST, the return type of function $bar(...)$ is unknown, which results in a false entity identification. When connecting changed entities, the type information is also important. Suppose in a scenario with multiple nested "CallExpressions" and "MemberExpressions", \codefont{module.member1.call1(...).member2.call2(...)}, since the return type of $call1(...)$ is unknown, we can't get the type information or generate the signatures of \codefont{member2} and \codefont{call2}, causing miss of syntactic dependency connections.

When the Typed-AST is applicable, the JSON-format ASTs can provide the inferred type for each token. For the first case mentioned above, \codefont{foo = bar(...)} where \codefont{bar(...)} returns a function, Typed-AST can detect that \codefont{foo} is a function and gives all the binding information including the return type and parameter types. For the second case, \codefont{module.member1.call1.member2.call2}, Typed-AST provides the inferred type for all the members and callee functions, signatures can be sucessfully generated and no connections are going to be missed. However, Typed-AST can't parse out all the binding information since we didn't apply it to the whole project for each commit. Typed-AST is designed by r2c company to analyze the type information for an entire project, it uses "package.json" file as an entry to download all the library dependencies, and then outputs the typed JSON-format AST of each file in the project with inferred types for each token and entity. Since it needs to download all the libraries dependencies, applying it to the entire project is time-costing and resource-costing, especially when we have thousands of commits to analyze for each project. We handle this challenge by just putting the changed JavaScript files and the corresponding "package.json" file together in a folder and implementing Typed-AST on the folder for each commit. It's inevitable to miss some type binding information, and the inferred type of some tokens are going to be output as "any". When that happens, our signature system method is triggered for remedy. To summarize, the type information generated by Typed-AST is more precise than our signature systems both in the aspects of entity identification and entities connection. Our design of Change Distiller (Section~\ref{sec:changedistiller}) and Type Binding are shown in Figure~\ref{fig:typebinding}.

\begin{figure}
\centering
\vspace{0em}
	\includegraphics[width=8.5cm]{images/typebinding.pdf}
	%\vspace{-1em}
	\caption{Our binding design takes in both the old and  new versions of JavaScript files edited for a bug fix, and uses Esprima, Typed-AST, as well as GumTreeDiff tools to resolve bindings in separate versions.}	
	\label{fig:typebinding}
	\vspace{1.5em}
\end{figure}
	
\subsection{Design of Co-Change Suggester}
\label{sec:suggester}
In our empirical study, we analyzed 14747 bug fixes from 10 popular open source projects to explore multi-enity edits, including Node.js~\cite{node}, Meteor~\cite{meteor}, Ghost~\cite{ghost}, Habitica~\cite{habitica}, Pdf.js~\cite{pdf}, React~\cite{react}, Serverless~\cite{serverless}, Webpack~\cite{webpack}, Storybook~\cite{storybook}, and Electron~\cite{electron}. Our study shows that recurring change patterns commonly exists in all the projects (Section~\ref{sec:patterns}). In particular, \textbf{*CF$\rightarrow$CF} , \textbf{*CF$\rightarrow$AF}, and \textbf{*CF$\rightarrow$AV} are three of the most frequently applied patterns. We design \tool to suggest function co-changes to complete these three change pattern edits. Specifically, given a multi-entity edit that (i) changes a function or adds a new function or adds a new variable (ii) modifies one or more functions to access the variable or invoke the function, our tool suggests other functions to co-change for the variable access or function invocation.

For each AF (AV or CF), we constructed suggestion tasks by (i) providing the AF (AV or CF) and one of its co-applied CF as input, and (ii) using the remaining part as the oracle to evaluate our tool's output. For instance, suppose that a commit has an added function $f_n$ and two changed functions $F=\{f_1, f_2\}$. In one task, we provide $f_n$ and $f_1$ as input, and check whether \tool suggests $f_2$ for change. Alternatively, we can provide $f_n$ and $f_2$ as input, and check whether \tool's output is $f_1$. In this way, if a \textbf{*CF$\rightarrow$AF} edit has one AF and $n$ CFs ($n\ge 2$), we can create $n$ tasks based on the edit. In each task, only one AF and one CF are provided as input, and all the other CF(s) is/are treated as the expected output. 

We apply machine-learning techniques in our experiments under the category of \emph{classification learning}. In the classification learning we apply different induction algorithms to a set of pre-classified training examples of the concept we want to learn (e.g., relations between pairs of functions). The output of the induction algorithm is referred to as a \emph{binary classifier}, which is also known as a model or a \emph{concept description}. Each training example is a known or solved case of the concept we want to learn, in that it is assigned \emph{an outcome} or \emph{a class}. An example is described in terms of the observed values for a set of features or attributes. Once a model or classifier is learned from a set of training examples it can be used to predict the class or outcome of unclassified or unsolved examples, in our case the outcome is weather a candidate function should be co-changed or not, we name the two classes Relevant and Not-Relevant where Relevant means that a change in one function will likely result in a change of the other function. In Figure~\ref{fig:classifier} an induction algorithm reads $k$ pre-classified examples $e_1, ..., e_k$ of some concept we want to learn. Each sample $e_i$ is described by $n$ attributes, and is assigned a class which is Relevant or Non-Relevant (changed or unchanged). 

For each \textbf{*CF$\rightarrow$CF} , \textbf{*CF$\rightarrow$AF}, or \textbf{*CF$\rightarrow$AV} task, the samples are generated by Relevant function pairs $(f_1, f_2)$, $(f_2, f_1)$ and Non-Relevant function pairs $(f_1, f_{u})$, $(f_2, f_{u})$, where $f_1$ and $f_2$ are the co-changed functions to access the 1CF $f_n$, or 1AF $f_n$, or 1AV $v_n$, where $f_{u}$ are the unchanged functions. To reduce the number of potential Non-Relevant pairs, we rely on the visibility of $f_n$ or $v_n$. Specifically, if $f_n$ is a private function, only the functions declared in $f_n$'s declaring file $F$ are analyzed because $f_n$ is invisible to any function outside $F$. Similarly, if $f_n$ is declared in $F$ and exported as a property of module $F$, then we scan all unchanged functions in the project. Another case is that $f_n$ is declared in the module export statement, then we only scan all the other files excluding $F$. 


\subsection{Attributes used in the experiments}
\label{sec:attributes}
Each sample of the co-change relation, that holds between a pair of functions labeled as Relevant or Non-Relevant, must be described in term of a set of features. The attributes or features can be based on a property of one of the functions in the pair but more often are the similarities between the pair of functions. In general, the attribute sets contain syntactic attributes, semantic attributes, token and statements based attributes and historic co-change record attributes.

Syntactic attributes are based on syntactic constructs in the source code as function calls, or data flow information such as variable or type definitions. As we will discuss in the preliminary study (Section~\ref{sec:preliminary}), co-changed functions usually access existing variables or invoke existing functions in common. We define two attributes here: \textbf{\emph{Number of common peer variables}} and \textbf{\emph{Number of common peer functions}}. Given an entity $e_n$ (e.g., $f_n$, $v_n$), we use \textbf{peer variables} to denote the existing variables that are (1) declared in the same file as $e_n$, and (2) accessed by one or more changed functions that also access $e_n$. Similarly we use \textbf{peer functions} to refer to the existing functions that are (1) declared in the same file as $e_n$, and (2) invoked by one or more changed functions which also access $e_n$. Our tool traverse the AST of each changed fucntion's old version to extract the accessed existing variables and the invoked existing functions, extracting a peer variable set $PV=\{pv_1,pv_2,\ldots\}$ and a peer function set $PF=\{pf_1,pf_2,\ldots\}$. Then common peer variable set and common peer function set can be generated by intersecting the peer variable sets of the function pairs and peer function sets of the function pairs.

Semantic attributes are based on the type information of the pair of functions. Intuitively, \emph{if a function should be changed to invoke $f_n$, this function is likely to contain the related calling context, i.e., properly typed variables that (1) pass values to $f_n$ as parameters or (2) accept values returned by $f_n$.} With this intuition, for any candidate function $f_c$, our tool traverses the AST of $f_c$ to extract the list of used types $L_{type}$. Such type information is mined from the type binding of any local variable used in $f_c$. And then we calculate the \textbf{\emph{Number of parameter types}} that both exist in $L_type$ and the parameter set of $f_n$ as an attribute. Another attribute is whether $f_c$ \textbf{\emph{Contains the return type}} of $f_n$. Similarly for a new variable $v_n$, we have the same attribute weather $f_c$ \textbf{\emph{Contains the type}} of $v_n$. In addition to the relation between candidate functions $f_c$ and the newly added or changed entity, we are also interested in the semantic similarities between the pair of functions. We create attributes if the pairs have the \textbf{\emph{Same return type}} and how many \textbf{\emph{Common parameter types}} they shared. As we discussed in Section~\ref{sec:changedistiller}, a function can be declared in many ways, our last semantic attribute is whether the pairs have the \textbf{\emph{Same declaration kind}}. For example, if the function pairs are declared as methods in the same class, then it's more possible for them to co-change together to access a newly added variable or function in the class.

The similarity between the pair of functions can also be indicated by the commonality of their tokens and statements. As we will discuss in Section~\ref{sec:preliminary}, a large percentage of co-changed functions have similar statements, and those similar statements usually change together for a bug fix. To calculate the attribute \textbf{\emph{Token similarity}}, we use the same way as we identify expression changes discussed in Section~\ref{sec:changedistiller} by calculating the percentage of the longest common token subsequence. To extract the attribute \textbf{\emph{Statement similarity}},
we ignore the sequence of the statements, just use the percentage of the common statements, i.e., $number\  of\  common \ statements \ *\  2 /\  number \ of\  total \ statements$.

To increase the accuracy of our classifier, we add an attribute \textbf{\emph{Historical record}} which illustrates how many times the pair of functions have changed together prior to the current commit. In Section~\ref{sec:compare} we will discuss how ROSE~\cite{Zimmermann:2004} mines the association rules between co-changed entities from software version histories. By adding this attribute, we are assuming \tool is a not only syntactic/semantic based tool but also history based classifier. All the attributes discussed above are listed in Table~\ref{tab:features}.

Notice that all the attributes that are related to type information (2nd to 6th in the list) are generated by Typed-AST. We already discussed that Node.js can't be parsed by Typed-AST due to the lack of npm dependency. So the training data set for Node.js only has 6 attributes for the 3 patterns. The other projects have 10 attributes for \textbf{*CF$\rightarrow$CF} and \textbf{*CF$\rightarrow$AF} patterns, and 9 attributes for \textbf{*CF$\rightarrow$AV} pattern (number of parameter types is excluded since an added variable doesn't have parameters).

%\begin{wraptable}{r}{8.7cm}
\begin{table}
	\centering
	%\vspace{-0.5em}
	\caption{Attribute List}
	\vspace{-0.5em}
	\label{tab:features}
	%\scriptsize
	\footnotesize
	\resizebox{\columnwidth}{!}{%
	\begin{tabular}{L{4.5cm}|L{2cm}}
		\toprule
		\textbf{Attribute Name} & \textbf{Attribute Type} \\
		\toprule
		% \# of fixes with the pattern *CM$\rightarrow$AF & 28 & 83 & 61 & 15\\
		% \midrule
		\# of common peer variables & Integer\\
		\midrule
		\# of common peer functions & Integer\\
		\midrule
		\# of parameter types & Integer\\
		\midrule
		Contains return type & Boolean\\
		\midrule
		Same return type & Boolean\\
		\midrule
		\# of common parameter types & Integer\\
		\midrule
		Same declaration kind & Boolean\\
		\midrule
		Token similarity & Double\\
		\midrule
		Statement similarity & Double\\
		\midrule
		Historical record & Integer\\
		\bottomrule
	\end{tabular}}
	\vspace{-0.5em}
\end{table}
%\end{wraptable}

\subsection{Machine-learning models used in the experiments}
\label{sec:models}
We performed classification by using Weka~\cite{weka}, a collection of machine learning algorithms for data mining tasks. To implement \tool, We applied four different classification algorithms built in Weka: Random forest~\cite{RandomForest}, J48 decision tree~\cite{j48}, Adaboost.M1~\cite{adaboost}, and Naive Bayes.

\begin{itemize}
    \item  Random forest classifier consists of a combination of tree classifiers where each classifier is generated using a random vector sampled independently from the input vector. The "forest" it builds, is an ensemble of decision trees, usually trained with the “bagging” method. The general idea of the bagging method is that a combination of learning models increases the overall result. To simplify, random forest builds multiple decision trees and merges them together to get a more accurate and stable prediction. In our implementation, we set the tree numbers to 100.
    \item J48 decision tree (C4.5) is an algorithm used to generate a decision tree developed by Ross Quinlan. C4.5 is an extension of Quinlan's earlier ID3~\cite{ID3} algorithm. The decision trees generated by C4.5 can be used for classification, and for this reason, C4.5 is often referred to as a statistical classifier. C4.5 builds decision trees from a set of training data in the same way as ID3, using the concept of information entropy. At each node of the tree, C4.5 chooses the attribute of the data that most effectively splits its set of samples into subsets enriched in one class or the other. 
    \item AdaBoost is best used to boost the performance of decision trees on binary classification problems. It was  originally called AdaBoost.M1 by the authors of the technique Freund and Schapire. More recently it may be referred to as discrete AdaBoost because it is used for classification rather than regression. AdaBoost.M1 is best used with weak learners. The most suited and therefore most common algorithm used with AdaBoost are decision trees with one level. Because these trees are so short and only contain one decision for classification, they are often called decision stumps. The final classifier of AdaBoost.M1 is a linear combination of weak decision tree stumps.
    \item Naive Bayes classifiers are classifiers with the assumption that features are statistically independent of one another. Unlike many other classifiers which assume that, for a given class, there will be some correlation between features, naive Bayes explicitly models the features as conditionally independent given the class. Because of the independence assumption, naive Bayes classifiers are highly scalable and can quickly learn to use high dimensional features with limited training data. 
\end{itemize}

To evaluate each classifier's performance, we applied 10-fold cross validation technique. As we discussed in~\ref{sec:suggester}, for co-changed functions $f_1$ and $f_2$, both pairs $(f_1, f_2)$ and $(f_2, f_1)$ are generated in the data set. Since most of the attributes represent the relations between $f_1$ and $f_2$, the data samples for the two pairs are very similar. To avoid similar samples appearing in the same data set (e.g., training set, testing set), we pre-sorted our data sets for each project to put pairs $(f_1, f_2)$ and $(f_2, f_1)$ neighboring each other, and disabled cross validation's shuffling and stratification functionalities that could shuffle the already sorted data set. We evaluate the performance of our tool for each project separately. Our design and evaluation of \tool is shown in Figure~\ref{fig:classifier}.

\begin{figure}
\centering
\vspace{0em}
	\includegraphics[width=8.5cm]{images/classifier_eval.pdf}
	%\vspace{-1em}
	\caption{Design and evaluation of our machine-learning based CF suggester.}	
	\label{fig:classifier}
	\vspace{1.5em}
\end{figure}


==> results.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Empirical Results}
\label{sec:empirical_result}
In this section, we first introduce the subject projects used
in our study (Section~\ref{sec:projects}), and then discuss our findings for the research questions (Sections~\ref{sec:frequency},~\ref{sec:patterns}, and ~\ref{sec:preliminary}).

\subsection{Subject Projects}
\label{sec:projects}
In our study, we leveraged the multi-entity edits of ten open-source projects:
\begin{itemize}
\item \emph{Node.js~\cite{node}} is a platform built on Chrome's JavaScript runtime for easily building fast and scalable network applications.

\item \emph{Meteor~\cite{meteor}} is a leading open source isomorphic Javascript framework designed to build scalable web, mobile and desktop apps quickly and efficiently. 

\item \emph{Ghost~\cite{ghost}} is one of the world's most popular modern open source publishing platforms. It is a headless Node.js CMS used by Apple, Sky News, Tinder and thousands more.

\item \emph{Habitica~\cite{habitica}}, formerly HabitRPG, is an online task management application run by HabitRPG, Inc. Unlike most task management programs, Habitica takes the form of a role-playing game. 

\item \emph{Pdf.js~\cite{pdf}} is A general-purpose, web standards-based platform for parsing and rendering PDFs.

\item \emph{React~\cite{react}} is a JavaScript library for building user interfaces. It is maintained by Facebook and a community of individual developers and companies. React can be used as a base in the development of single-page or mobile applications.

\item \emph{Serverless~\cite{serverless}} is a free and open-source web framework written using Node.js. Serverless is the first framework developed for building applications on AWS Lambda, a serverless computing platform provided by Amazon as a part of Amazon Web Services.

\item \emph{Webpack~\cite{webpack}} is an open-source JavaScript module bundler. It is a module bundler primarily for JavaScript, but it can transform front-end assets like HTML, CSS, and images if the corresponding loaders are included. 

\item \emph{Storybook~\cite{storybook}} is an open source tool for developing UI components in isolation for React, Vue, and Angular. It makes building stunning UIs organized and efficient.

\item \emph{Electron~\cite{electron}} is an open-source framework developed and maintained by GitHub. Electron allows for the development of desktop GUI applications using web technologies: It combines the Chromium rendering engine and the Node.js runtime.
\end{itemize}
These projects have well-maintained version control systems and very few JavaScript files that are constructed by using the Asynchronous Module Definition (AMD) API, which our tool doesn't support due to its complicated construction. In this paper, we mainly focus on the program commits that fix bugs. Therefore, we collected bug-fixing commits based on the keywords like “bug”, “fix”, "error", "failure", and "adjust" in commit messages.
TABLE~\ref{tab:projects} presents more information about these projects.
KLOC shows the code size of each project. \# of Fixes shows
each project’s total number of bug fixes that can be processed by our tool.
All our following investigations are based on these 14747 fixes. \#
of Entity Changes reports the number of entity changes we
extracted from these fixes.

%\begin{wraptable}{r}{8.7cm}
\begin{table}
	\centering
	%\vspace{-0.5em}
	\caption{Subject projects}
	\vspace{-0.5em}
	\label{tab:projects}
	%\scriptsize
	\footnotesize
	\resizebox{\columnwidth}{!}{%
	\begin{tabular}{L{1.5cm}|R{1cm}|R{1.2cm}|R{1.5cm}}
		\toprule
		\textbf{Projects} & \textbf{KLOC} & \textbf{\# of Fixes} & \textbf{\# of Entity Changes}\\
		\toprule
		% \# of fixes with the pattern *CM$\rightarrow$AF & 28 & 83 & 61 & 15\\
		% \midrule
		Node.js & 1755 & 2701 & 11287\\
		\midrule
		Metoer & 255 & 3011 & 10274\\
		\midrule
		Ghost & 115 & 1263 & 5142\\
		\midrule
	    Habitica & 129 & 1858 & 6116\\
		\midrule
		Pdf.js & 104 & 1754 & 4255\\
		\midrule
		React & 286 & 1050 & 4415\\
		\midrule
	    Serverless & 63 & 1110 & 3846\\
		\midrule
		Webpack & 37 & 1099 & 3699\\
		\midrule
		Storybook  & 43 & 528 & 2277\\
		\midrule
		Electron & 35 & 673 & 1898\\
		\bottomrule
	\end{tabular}}
	\vspace{-0.5em}
\end{table}
%\end{wraptable}

\subsection{Properties of Multi-Entity Edits}
\label{sec:frequency}
Form all the changed entities we extracted, We are interested in \emph{what is the frequency of multi-entity bug fixes}? This question examines the prevalence of multi-entity changes in real fixes, and explores the syntactic dependence relations between co-changed entities. 

As shown in Figure~\ref{fig:change_distribution}, the extracted changes distribute unevenly among the eleven predefined change types, and different projects have different relative distributions of the change types. For instance, Node.js and Serverless have 51\% and 66\% changed entities as \textbf{CF}s, whereas Storybook and React only have 16\% and 18\% changed entities as \textbf{CF}s. Meteor, Habitica and Electron have more than 30\% changed entities as \textbf{CE}s, accounting for the largest portion for them. It's obvious that JavaScript programmers have different programming styles for different projects, and they change their styles when new ES features are released. For example, Serverless and Pdf.js are using more and more ES6 classes, whereas Node.js and Meteor are still using the strict mode and objected functions. Among all the changed entities, on average, \textbf{CF}s account for 33.5\%, \textbf{CE}s account for 12.8\%, both \textbf{AVs} and \textbf{AFs} account for 10.3\% of the changing types. These observations indicate that in addition to \textbf{CF}s and \textbf{CE}s, developers also frequently applied \textbf{AV}s and \textbf{AF}s to fix bugs.

\begin{figure*}
\centering
\vspace{0em}
	\includegraphics[width=\textwidth]{images/change_distribution.pdf}
	%\vspace{-1em}
	\caption{Change distribution among different change types}	
	\label{fig:change_distribution}
	\vspace{1.5em}
	\end{figure*}

We then clustered bug fixes according to the numbers of changed entities, we presented the results for four picked projects in Figure~\ref{fig:distribution}. Among the ten projects, 41-52\% of the fixes involve multi-entity changes. Specifically, 15-19\% of the fixes include two-entity changes, and 7-10\% of the fixes involve three-entity changes. We found the number of fixes decreases with the increasing number of changed entities. The maximum number of changed entities appears in Node.js, where a single fix modifies 335 entities. We manually checked the commit on GitHub~\cite{e71e71b}, and found in that commit, four important JavaScript files were added and three other JavaScript files were changed to implement HTTP/2. 

\begin{figure*}
\centering
\vspace{0em}	\includegraphics[width=\textwidth]{images/distribution.pdf}
	%\vspace{-1em}
	\caption{Bug fix distribution based on the number of included changed entities}	
	\label{fig:distribution}
	\vspace{1.5em}
	\end{figure*}

\begin{figure*}
\centering
\vspace{0em}
	\includegraphics[width=\textwidth]{images/cdg.pdf}
	%\vspace{-1em}
	\caption{ The distribution of fixes with CDG(s) based on the number of extracted CDGs}	
	\label{fig:cdg}
	\vspace{1.5em}
	\end{figure*}


Among the fixes with multi-entity edits, we further clustered these bug fixes based on the number of CDG(s) built for them. As shown in Table~\ref{tab:CDGs}, \textbf{\# of Fixes with Multi-Entity Edits} shows the number of fixes containing at least two changed entities. \textbf{\# of Fixes with CDG(s) Extracted} indicates the number of fixes for which we built at least one CDG based on the analyzed syntactic dependence relationship between changed entities. Then we calculated the \textbf{\% of Fixes with CDG(s) Extracted} from those multi-entity edits. We found that averagely 49.4\% of the multi-entity edits contain at least one CDG, which shows that JavaScript developers usually change related entities together to fix bugs. Because our incomplete program analysis may miss some type identifications and dependencies between co-changed entities due to the limited analysis scope (i.e., changed sourse files only), the actual percentage of related co-changes should be higher than our reported values. 

%\begin{wraptable}{r}{8.7cm}
\begin{table}
	\centering
	%\vspace{-0.5em}
	\caption{Bug fixes with multi-entity changes}
	\vspace{-0.5em}
	\label{tab:CDGs}
	%\scriptsize
	\footnotesize
	\resizebox{\columnwidth}{!}{%
	\begin{tabular}{L{1.2cm}|R{1.5cm}|R{1.5cm}|R{1.5cm}}
		\toprule
		\textbf{Projects} & \textbf{\# of Fixes with Multi-Entity Edits} & \textbf{\# of Fixes with CDG(s) Extracted} & \textbf{\% of Fixes with CDG(s) Extracted}\\
		\toprule
		% \# of fixes with the pattern *CM$\rightarrow$AF & 28 & 83 & 61 & 15\\
		% \midrule
		Node.js & 1401 & 785 & 56.0\%\\
		\midrule
		Metoer & 1445 & 670 & 46.4\%\\
		\midrule
		Ghost & 604 & 356 & 58.9\%\\
		\midrule
	    Habitica & 962 & 345 & 35.9\%\\
		\midrule
		Pdf.js & 711 & 372 & 52.3\%\\
		\midrule
		React & 538 & 320 & 59.5\%\\
		\midrule
	    Serverless & 480 & 171 & 35.6\%\\
		\midrule
		Webpack & 483 & 253 & 52.4\%\\
		\midrule
		Storybook  & 243 & 119 & 49.0\%\\
		\midrule
		Electron & 277 & 123 & 44.4\%\\
		\bottomrule
	\end{tabular}}
	\vspace{-0.5em}
\end{table}
%\end{wraptable}

We further clustered the fixes based on the number of CDGs extracted. As shown in Figure~\ref{fig:cdg}, we found that as the number of CDGs increases, the number of fixes goes down. Specifically, 73\%-81\% of such fiexes contain single CDG, 9\%-18\% of the fixes contain two CDGs, and 3\%-7\% of the fixes have three CDGs. The fix containing the largest number of CDGs (i.e. 16) is the one with the maximum number of changed entities in Node.js as discussed above. Similar fact has been concluded in our prior work of the empirical study for bug fixes in Java projects~\cite{ye2018}. With the CDGs extracted, we can visualize relationship between changes across entities, which helped us to design \tool. However, current diff tools only compare code by text (e.g., UNIX diff~\cite{unixdiff}), ASTs (e.g., ~\cite{Falleri2014:GumTree}), without giving the syntactic relations between those co-changed parts.

\subsection{Patterns of Multi-Entity Edits}
\label{sec:patterns}
In this section, we are going to explore the recurring co-change patterns in real bug fixes, and identify the most frequent patterns among all projects.

We have defined recurring change patterns in Section~\ref{sec:concepts}. Suppose we compared CDGs pair-by-pair and identified patterns presented as $RCP = \{rcp_1, rcp_2, ..., rcp_s\}$. We calculated a pattern's frequency by further matching the pattern with all commits' CDGs to count how many times it appears as a subgraph of a CDG. Notice that if two patterns (e.g., $rcp_p$ and $rcp_q$) find matches in the same CDG, and on pattern is a subgraph of the other (e.g., $rcp_p$ is contained in $rcp_q$), we will only count the occurrence of the larger pattern (e.g., $rcp_q$) to avoid double counting overlapped patterns.

Table~\ref{tab:patterns} shows the number of recurring change patterns identified in 10 projects is in the range of 35-221. We counted the number of fixes matching these patterns for each project, and if we compare these numbers against the \textbf{\# of Fixes with CDG(s) Extracted} in Table~\ref{tab:CDGs}, it's showing that almost every fix with CDG(s) extracted contains at least one subgraph matching a pattern. We also counted the number of subgraphs that matches the patterns, we found that there are more matched subgraphs than matched fixes, indicating that many fixes contain multiple matched subgraphs.

%\begin{wraptable}{r}{8.7cm}
\begin{table}
	\centering
	%\vspace{-0.5em}
	\caption{Recurring change patterns and their matches}
	\vspace{-0.5em}
	\label{tab:patterns}
	%\scriptsize
	\footnotesize
	\resizebox{\columnwidth}{!}{%
	\begin{tabular}{L{1.2cm}|R{1.5cm}|R{1.5cm}|R{1.5cm}}
		\toprule
		\textbf{Projects} & \textbf{\# of Patterns} & \textbf{\# of Fixes Matching the Patterns} & \textbf{\# of Subgraphs Matching the Patterns}\\
		\toprule
		% \# of fixes with the pattern *CM$\rightarrow$AF & 28 & 83 & 61 & 15\\
		% \midrule
		Node.js & 221 & 782 & 2385\\
		\midrule
		Metoer & 200 & 658 & 1719\\
		\midrule
		Ghost & 133 & 351 & 1223\\
		\midrule
	    Habitica & 116 & 339 & 706\\
		\midrule
		Pdf.js & 86 & 367 & 640\\
		\midrule
		React & 110 & 316 & 899\\
		\midrule
	    Serverless & 57 & 164 & 372\\
		\midrule
		Webpack & 80 & 243 & 583\\
		\midrule
		Storybook  & 42 & 113 & 337\\
		\midrule
		Electron & 35 & 117 & 228\\
		\bottomrule
	\end{tabular}}
	\vspace{-0.5em}
\end{table}
%\end{wraptable}

We accumulated the recurring change patterns for different projects and identified five most popular recurring change patterns by counting the fixes that match the patterns, as shown in Figure~\ref{fig:popular}. The top three patterns commonly exist in all 10 projects, while the other two don't. 

\begin{figure}
\centering
\vspace{0em}
	\includegraphics[width=8.5cm]{images/popular.pdf}
	%\vspace{-1em}
	\caption{Five most popular recurring change patterns among the 10 projects}	
	\label{fig:popular}
	\vspace{0em}
\end{figure}

\begin{itemize}
    \item[\textbf{P1:}] \emph{A callee function experiences a \textbf{CF} change, while one or more of its caller functions also experience \textbf{CF} changes.}  We present this pattern as \textbf{*CF$\stackrel{f}\rightarrow$CF}, where the \textbf{*CF} node means one or more caller functions, the \textbf{CF} node represents the callee function, and the \textbf{f}-annotated edge shows the caller-callee relationship, e.g., function invocation here. The edge's direction represents the invocation direction. This pattern is the most popular one, it exists in 218 fixes in Node.js, 152 fixes in Meteor, 104 fixes in Pdf.js, etc.. Programmers would like to change on callee function together with the function's caller(s) to fix bugs. 
    
    \item[\textbf{P2:}] \emph{A module or a class experiences an \textbf{AF} change, while one or more other functions go through \textbf{CF} changes.} This pattern is presented as \textbf{*CM$\stackrel{f}\rightarrow$AM}, where the \textbf{*CF} node still means one or more changed caller functions, the \textbf{AF} node represents one added function, and the \textbf{f}-annotated edge shows the caller-callee relationship. As the second most common pattern, it appears in 128 fixes in Node.js, 83 fixes in Meteor, and 69 fixes in Webpack, etc.. Intuitively, when developers add a new function to fix a bug, they usually modify existing functions(s) to invoke the new function. 
    
    \item[\textbf{P3:}] \emph{A module or a class experiences an \textbf{AV} change, while one ore more functions accessing the variable experience \textbf{CF} changes.} We denote this pattern as \textbf{*CF$\stackrel{v}\rightarrow$AV}, where the \textbf{AV} node represents one added variable, and the \textbf{v}-annotated edge shows the variable access relationship between a variable and a function. As the third most common pattern, it appears in 114 fixes in Node.js, 59 fixes in Ghost, and 53 fixes in Meteor, etc.. It's apparent that developers usually modify existing functions(s) to access an added variable.
    
    \item[\textbf{P4:}] \emph{A variable experiences an \textbf{AV} change, while one or more functions accessing the variable undergo \textbf{AF} changes.} Similarly, we use \textbf{*AF$\stackrel{v}\rightarrow$AV} to present this pattern. As the fourth most popular recurring change pattern, it only shows up in 9 out of 10 projects, with meteor as an exception. This pattern appears in 68 fixes in Node.js, 60 fixes in Ghost, and 36 fixes in React, etc.. Intuitively, when developers add a variable to fix a bug, they may also add one or more new functions to access the variable.
    
    \item[\textbf{P5:}] \emph{A function experiences a \textbf{CF} change, while one or more expressions accessing the function undergo \textbf{CE} changes,} which is represented as \textbf{*CE$\stackrel{f}\rightarrow$CF}, where the \textbf{*CE} node means one or more changed expressions. This pattern only exists in three projects : Meteor (81 fixes), Habitica (43 fixes), and Electron (20 fixes), since these three projects have more than 30\% changed entities as \textbf{CE}s, as mentioned in Section~\ref{sec:frequency} and shown in Figure~\ref{fig:change_distribution}. Intuitively, when a project contain lots of expressions to implement some functionalities, developers usually change those expression(s) that invoked one changed callee function to fix bugs.
\end{itemize}

\subsection{Preliminary Study}
\label{sec:preliminary}
We are curious why programmers make multi-entity edits when they fix real bugs. We conducted preliminary study to analyze some fixes matching the top 3 patterns by checking for the content and context of the recurring change patterns. In the study, we manually examined 20 fixes for each pattern from P1-P3, where multiple functions co-change together for the changed function invocation (P1), new function invocation (P2) and new variable access (P3), we inspected these 60 fixes to investigate any characteristics and commonalities between the co-changed functions. For example, we use "FI" to present that co-changed functions invoke the same set of peer functions, "VA" to present that they access the same set of peer variables, "ST" and "SS" to present that they have similar tokens and statements, where the identical parts should account for at least 50\%.

Table~\ref{tab:inspect_P1}, ~\ref{tab:inspect_P2} and ~\ref{tab:inspect_P3} present our inspection results for P1, P2, and P3 edits respectively. For each pattern, about 2-5 or 2-6 functions co-changed to access a variable or invoke a function. For pattern P1 (Table~\ref{tab:inspect_P1}), only in 4 out of 20 examined revisions the co-changed functions have nothing in common. \textbf{In 9 out of 20 examined revisions, the co-changed functions commonly invoke existing method(s) before the edits are applied};  whereas the other 6 commits have co-changed functions either to commonly access certain variable(s) or to share similar tokens and statements. For pattern P2 (Table~\ref{tab:inspect_P2}), \textbf{12 of the 20 revisions have co-changed methods sharing the same function invocation}, and only 2 commits share no commonality. \emph{Our finding shows that when one or more methods in a cluster are changed to invoke a new function (pattern P2) or for a callee function change (pattern P1), the other methods from the same cluster are likely to be co-changed for the new function invocation (P2) or for the callee function change (P1).} For pattern P3 (Table~\ref{tab:inspect_P3}), 3 out of 20 fixes have nothing in common; \textbf{in 13 commits, the co-changed functions commonly access existing variable(s) before the edits are applied}; while the other 4 revisions either share the same function invocation(s) or have similar tokens and statements. \emph{Our observation indicates that when one or more functions in a cluster are changed to access a new variable, the other functions from the same cluster are likely to be co-changed for the new variable access.} The findings are consistent with our prior work CMSuggester \cite{Jiang2020, Wang2018CMSuggester} for Java co-change suggestion.



\begin{table}
	\centering
	%\vspace{-5.5em}
	\caption{Commonality inspection of 20 \textbf{*CF$\rightarrow$CF} multi-entity edits}
	\label{tab:inspect_P1}
	%\vspace{-0.5em}
	\footnotesize
	%\small
%	\resizebox{\columnwidth}{!}{%
	\begin{tabular}{L{1.2cm}| l L{1.8cm} R{1.5cm} L{1.6cm}}
		\toprule
		\textbf{Project} & \textbf{Commits} & \textbf{Changed Callee Function} & \textbf{\# of Changed Functions} & \textbf{Commonality}\\
		\toprule
		Node.js & 71203f5%~\cite{aries3d072a4}
		& getActual(...) & 2 & FI, ST \\ \cline{2-5}
		&  d75f67f%~\cite{aries50ca3da}
		& fail(...) & 6
		& FI, VA\\ \cline{2-5}
		&  9a6dd07%~\cite{aries5d334d7}
		& processList(...) & 2
		& None \\ \cline{2-5}
		& 69e6c5a%~\cite{aries95766a2}
		& request(...) & 2
		& VA\\ \cline{2-5}
		& f2ec46a%~\cite{aries9586d78}
		& pause(...) & 3
		& FI\\ %\cline{2-5}
		\midrule
		Meteor & 5568709%~\cite{cas0792766}
		& makeObjectLiteral(...) & 2
		& FI, ST\\ \cline{2-5}	
		&  64d939a%~\cite{cas0963469}
		& refresh(...) & 2
		& FI \\ \cline{2-5}
		&  0ad0083%~\cite{cas0d1d3bc}
		& \_returnFirst(...) & 5
		& ST, SS\\ \cline{2-5}
		& 06a7dc9%~\cite{cas1c9c47d}
		& getLoadedPackageVersions(...)& 2
		& VA\\ \cline{2-5}
		& 3e60740%~\cite{cas266e94f}
		& \_buildTimeDirectDependenciesWithBuildIds(...) & 4
		& FI, VA\\ %\cline{2-5}
		\midrule
		Ghost & 5d028b7%~\cite{derby-099e28f}
		& apiRoutes(...) & 2
		& None\\ %\cline{2-5}
		\midrule
		Habitica & 6fcf739%~\cite{derby-099e28f}
		& exportEntity(...) & 2
		& ST, SS\\ %\cline{2-5}
		\midrule
		Pdf.js & 9a47a86%~\cite{derby-f578f070}
		& \_setCurrentPageNumber(...)& 3
		& None\\ \cline{2-5}
		& 2fe9f3f%~\cite{derby-6eb5042}
		& Ref(...)&3
		& FI\\ \cline{2-5}
		& b76cf66%~\cite{derby-2f41733}
		& CFFparser(...)& 3
		& FI \\ %\cline{2-5}
		\midrule
		React & ea089fd%~\cite{derby-099e28f}
		& \_assertSingleLink(...) & 2
		& ST\\ %\cline{2-5}
		\midrule
		Serverless & a933846%~\cite{derby-099e28f}
		& getEndpoints(...) & 2
		& ST, SS\\ %\cline{2-5}
		\midrule
		Webpack & e0f975e%~\cite{derby-099e28f}
		& allHaveModule(...) & 2
		& None\\ %\cline{2-5}
		\midrule
		Storybook & 46a5f1a%~\cite{derby-099e28f}
		& createPreviewEntry & 2
		& ST, SS\\ %\cline{2-5}
		\midrule
		Electron & 6f5b0a2%~\cite{derby-81b9853}
		& \_write(...)& 2
		& VA\\ %\cline{2-5}
		\bottomrule
	\end{tabular} %}
	\vspace{-.5em}
\end{table}

\begin{table}
	\centering
	%\vspace{-5.5em}
	\caption{Commonality inspection of 20 \textbf{*CF$\rightarrow$AF} multi-entity edits}
	\label{tab:inspect_P2}
	%\vspace{-0.5em}
	\footnotesize
	%\small
%	\resizebox{\columnwidth}{!}{%
	\begin{tabular}{L{1.2cm}| l L{1.8cm} R{1.5cm} L{1.6cm}}
		\toprule
		\textbf{Project} & \textbf{Commits} & \textbf{Added Function} & \textbf{\# of Changed Functions} & \textbf{Commonality}\\
		\toprule
		Node.js & 62e0ca0%~\cite{aries3d072a4}
		& pause(...) & 2 & FI\\ \cline{2-5}
		&  3398cce%~\cite{aries50ca3da}
		& chunkify(...) & 2
		& FI, VA\\ \cline{2-5}
		& 81bc23f%~\cite{aries5d334d7}
		& formatSetIterInner(...) & 2
		& FI, ST, SS \\ \cline{2-5}
		& 481329e%~\cite{aries95766a2}
		& killChild(...) & 2
		& FI, VA\\ \cline{2-5}
		& df33d8d%~\cite{aries9586d78}
		& validateSettings(...) & 3
		& VA, ST\\ %\cline{2-5}
		\midrule
		Meteor & 5568709%~\cite{cas0792766}
		& cleanUpTimer(...) & 2
		& VA\\ \cline{2-5}	
		& 0ad0083%~\cite{cas0963469}
		& \_getPackage(...) & 2
		& ST, SS \\ \cline{2-5}
		& 8bcbd65%~\cite{cas0d1d3bc}
		& mapWhereToArch(...) & 2
		& FI, VA\\ \cline{2-5}
		& 21f976d%~\cite{cas1c9c47d}
		& processBatches(...)& 2
		& FI, VA, ST\\ \cline{2-5}
		& 13f5d18%~\cite{cas266e94f}
		& sessionMethodCaller(...) & 2
		& FI\\ %\cline{2-5}
		\midrule
		Ghost & 7eb316b%~\cite{derby-099e28f}
		& attach(...) & 2
		& SS, ST\\ %\cline{2-5}
		\midrule
		Habitica & f1e200c%~\cite{derby-099e28f}
		& pathExistsInArray(...) & 3
		& ST\\ %\cline{2-5}
		\midrule
		Pdf.js & 6f67e39%~\cite{derby-2f41733}
		& replaceTemporaryNonWebpackRequireHack(...)& 4
		& FI, SS, ST \\ %\cline{2-5}
		\midrule
		React & 21d0c11%~\cite{derby-099e28f}
		& getImportSideEffects(...) & 2
		& None\\ %\cline{2-5}
		\midrule
		Serverless & dc3a4aa%~\cite{derby-099e28f}
		& populateObjectImpl(...) & 2
		& FI\\ %\cline{2-5}
		\midrule
		Webpack & 8bca2dc%~\cite{derby-f578f070}
		& ImportEagerWeakContextDependency(...)& 2
		& None\\ \cline{2-5}
		& 23d28dd%~\cite{derby-6eb5042}
		& getRenameIdentifier(...)&3
		& FI, SS\\ \cline{2-5}
		& e04b1a5%~\cite{derby-099e28f}
		& inBlockScope(...) & 5
		& FI\\ %\cline{2-5}
		\midrule
		Storybook & 838730f%~\cite{derby-099e28f}
		& renderErrorDisplay(...) & 2
		& ST\\ %\cline{2-5}
		\midrule
		Electron & 3094f62%~\cite{derby-81b9853}
		& getOwnerKey(...)& 3
		& FI, VA, SS\\ %\cline{2-5}
		\bottomrule
	\end{tabular} %}
	\vspace{.5em}
\end{table}

\begin{table}
	\centering
	\vspace{0.5em}
	\caption{Commonality inspection of 20 \textbf{*CF$\rightarrow$AV} multi-entity edits}
	\label{tab:inspect_P3}
	%\vspace{0.5em}
	\footnotesize
	%\small
%	\resizebox{\columnwidth}{!}{%
	\begin{tabular}{L{1.2cm}| l L{1.8cm} R{1.5cm} L{1.6cm}}
		\toprule
		\textbf{Project} & \textbf{Commits} & \textbf{Changed Callee Function} & \textbf{\# of Changed Functions} & \textbf{Commonality}\\
		\toprule
		Node.js & 71203f5%~\cite{aries3d072a4}
		& NO\_EXCEPTION\_SENTINEL & 3 & FI \\ \cline{2-5}
		&  3398cce%~\cite{aries50ca3da}
		& \_header & 2
		& FI, VA\\ \cline{2-5}
		&  9a6dd07%~\cite{aries5d334d7}
		& processList(...) & 2
		& FI \\ \cline{2-5}
		& 69e6c5a%~\cite{aries95766a2}
		& kMaxStreams & 4
		& VA, SS\\ \cline{2-5}
		&  9e32c2e%~\cite{cas0963469}
		& BIND\_STATE\_BOUND & 2
		& FI, VA \\ \cline{2-5}
		&  3abfb56%~\cite{cas0d1d3bc}
		& WriteWrap & 2
		& FI, VA\\ \cline{2-5}
		& e22d0de%~\cite{cas1c9c47d}
		& child& 2
		& None\\ %\cline{2-5}
		\midrule
		Meteor & 711d367%~\cite{cas0792766}
		& \_source & 5
		& ST, SS\\ \cline{2-5}	
		& 9813345%~\cite{derby-6eb5042}
		& messages & 4
		& VA, ST\\ \cline{2-5}
		& 9bf291c%~\cite{derby-2f41733}
		& debugOnly & 3
		& FI, VA \\ %\cline{2-5}
		\midrule
		Ghost & 639c0d0%~\cite{derby-099e28f}
		& schemaTables & 2
		& VA, ST\\ \cline{2-5}
		& 7ebd104%~\cite{derby-6eb5042}
		& availableApps & 2
		& VA\\ \cline{2-5}
		& add4c6bc%~\cite{derby-2f41733}
		& filesToDelete& 3
		& None \\ %\cline{2-5}
		\midrule
		Habitica & 592cfef%~\cite{derby-099e28f}
		& apiv4Prefix & 2
		& VA, ST, SS\\ %\cline{2-5}
		\midrule
		Pdf.js & 1ded729%~\cite{derby-f578f070}
		& \_onUpdateTextLayerMatches& 2
		& VA\\ %\cline{2-5}
		\midrule
		React & 111731d%~\cite{derby-099e28f}
		& moduleTypes & 4
		& VA, SS\\ %\cline{2-5}
		\midrule
		Serverless & 22d56ec%~\cite{derby-099e28f}
		& fse & 4
		& SS, ST\\ %\cline{2-5}
		\midrule
		Webpack & 3eefb91%~\cite{derby-099e28f}
		& \_cachedSource & 2
		& None\\ %\cline{2-5}
		\midrule
		Storybook & 19da888%~\cite{derby-099e28f}
		& \_channel & 2
		& VA\\ %\cline{2-5}
		\midrule
		Electron & 6f5b0a2 %~\cite{derby-81b9853}
		& extraHeaders & 3
		& VA, ST\\ %\cline{2-5}
		\bottomrule
	\end{tabular} %}
	\vspace{-.5em}
\end{table}










==> rq3.tex <==
\subsection{Sensitivity to The Adopted ML Algorithm}
\label{sec:compare_models}

To understand how sensitive \tool is to the selection of ML algorithms, in addition to Adaboost (Random Forest), we also explored four other algorithms: J48~\cite{j48}, Random Forest~\cite{RandomForest}, Na\"ive Bayes~\cite{nb}, and Adaboost (default).

\begin{figure}
\begin{subfigure}{\linewidth}
\includegraphics[width=\linewidth]{images/ml-comparison-cf-cf.pdf}
\vspace{-2.5em}
\caption{The *CF$\xrightarrow{f}$CF data}
\end{subfigure}
\begin{subfigure}{\linewidth}
%\caption{ based on $CF\xrightarrow{f}CF$} data
\includegraphics[width=\linewidth]{images/ml-comparison-cf-af.pdf}
\vspace{-2.5em}
\caption{The *CF$\xrightarrow{f}$AF data}
\end{subfigure}
\begin{subfigure}{\linewidth}
%\caption{ based on $CF\xrightarrow{f}CF$} data
\includegraphics[width=\linewidth]{images/ml-comparison-cf-av.pdf}
\vspace{-2.5em}
\caption{The *CF$\xrightarrow{v}$AV data}
\end{subfigure}
\caption{Comparison between different ML algorithms on different data sets}
\label{fig:ml-comparison}
\end{figure}

\begin{itemize}
\item \textbf{J48} builds a decision tree as a predictive model to go from observations about an item (represented in the branches) to conclusions about the item's target value (represented in the leaves).
\item \textbf{Na\"ive Bayes} calculates the probabilities of hypotheses by applying Bayes' theorem with strong (na\"ive) independence assumptions between features.
\item \textbf{Random Forest} is an ensemble learning method that trains a model to make predictions based on a number of different models. Random Forest trains a set of individual models in a parallel way. Each model is trained with a random subset of the data. Given a candidate in the testing set, individual models make their separate predictions and Random Forest uses the one with the majority vote as its final prediction.
%For each candidate in the test set, Random Forest uses the class with the majority
\item \textbf{Adaboost} is also an ensemble learning method. However, different from Random Forest, Adaboost trains a bunch of individual models (i.e., weak learners) in a sequential way. Each individual model learns from mistakes made by the previous model. We tried two variants of Adaboost: (1) Adaboost (default) with decision trees as the weak learners, and (2) Adaboost (Random Forest) with Random Forests as the weak learners.
\end{itemize}


Figure~\ref{fig:ml-comparison} illustrates the effectiveness comparison when \tool adopts different ML algorithms. The three subfigures (Figure~\ref{fig:ml-comparison} (a)--(c)) separately present the comparison results on the data sets of *CF$\xrightarrow{f}$CF, *CF$\xrightarrow{f}$AF, and *CF$\xrightarrow{v}$AV. We observed similar phenomena in all subfigures. First, Adaboost (Random Forest) and Random Forest achieved very similar effectiveness, and both of them considerably outperformed the other algorithms. Second, compared with Random Forest, Adaboost (Random Forest) obtained better precision, better recall, better accuracy, but equal or slightly lower coverage; thus, we chose Adaboost (Random Forest) as the default ML algorithm used in \tool.
Third, among all data sets, Na\"ive Bayes obtained the lowest recall and accuracy rates; while Adaboost (default) obtained the lowest coverage rates.

Our results imply that although ensemble learning methods generally outperform other ML algorithms, their effectiveness also depends on (1) what weak learners are used and (2) how we organize weak learners. Between Adaboost (Random Forest) and Adaboost (default), the only difference exists in the used weak learner (Random Forest vs.~Decision Tree). Our evaluation shows that Random Forest helps improve Adaboost's performance when it is used as the weak learner. Additionally, between Random Forest and Adaboost (default), the only difference is how they combine decision trees as weak learners. Our evaluation shows that Random Forest outperforms Adaboost by
training weak learners in a parallel instead of sequential way.


\begin{tcolorbox}
	\textbf{Finding 3:}
	\emph{\tool is sensitive to the adopted ML algorithm. \tool obtained the lowest prediction accuracy when Na\"ive Bayes was used, but acquired the highest accuracy when Adaboost (Random Forest) was used.
	% outperformed ROSE in many 1AF1C tasks. This means that \toolaf complements ROSE by inferring co-changes from methods' common field accesses instead of from the history.
	}
\end{tcolorbox}
%The above evaluation shows that \tool outperformed ROSE when implementing the Random forest classification algorithm. We are also curious how Random forest compares with the other classifiers when recommending changes for the 3 patterns and 8 projects. Thus, we also applied \tool by using J48 decision tree, Adaboost.M1 (Desicion Stumps), and Naive Bayes classifiers to the data set shown in Table~\ref{tab:1a1c}.

%Table~\ref{tab:4models} presents the weighted average metrics of the 4 machine-learning models for each pattern. Random forest outperformed all the other three classifiers in terms of all metrics. Specifically, Random forest suggested changes for more than 80\% of those tasks, while J48 decision tree provided suggestions for about 60-70\% of those tasks, the average coverage of Naive Bayes is about 60\%-80\%, and AdaBoost.M1 only suggested about 50\% changes. Among the provided suggestions, random forest achieved 71\%, 76\% and 76\% accuracy for \textbf{*CF$\rightarrow$CF}, \textbf{*CF$\rightarrow$AF} and \textbf{*CF$\rightarrow$AV} patterns; J48 decision tree acquired 61\%, 65\% and 64\% accuracy for the 3 patterns; AdaBoost.M1 achieved 62\%, 66\% and 64\% accuracy; though the coverage of Naive Bayes is higher than AdaBoost.M1, the accuracy is only 53\%, 57\% and 56\% for the 3 patterns, the lowest among the 4 classifiers. All 4 classifiers performed better than ROSE in terms of precision, recall and accuracy, though the coverage of AdaBoost.M1 is as low as ROSE (about 50\%).

%Random forest consists of multiple single trees each based on a random sample of the training data. They are typically more accurate than single decision trees. In our evaluation, random forest beats J48 decision tree with 15\% higher coverage and 10\% higher accuracy. In Random forest, certain number (e.g., 100) of full sized trees are grown on different subsets of the training dataset, whereas Adaboost.M1 uses stumps (decision tree with only one split). So, Adaboost is basically a forest of stumps. These stumps are called weak learners. These weak learners have high bias and low variance, which results in low precision and recall, and low coverage correspondingly. Compared to the other 3 classifiers, Naive Bayes has the lowest accuracy, since it strongly relies on the independence assumptions between the attributes. In our attribute set, some attributes are kind of related, for instance, higher \textbf{\emph{token similarity}} often results in higher \textbf{\emph{statement similarity}}.

\begin{comment}
\begin{table}
	\centering
	\scriptsize
	%\footnotesize
	\vspace{1em}
	\caption{\tool's effectiveness when it uses different ML algorithms}
	%\vspace{1em}
	\label{tab:4models}
	%\resizebox{\columnwidth}{!}{%
	\begin{tabular}{C{1.2cm}|R{0.6cm} R{0.6cm} R{0.6cm} R{0.6cm} | R{0.6cm} R{0.6cm} R{0.6cm} R{0.6cm}}
		\toprule
		\multirow{2}{*}{\textbf{Pattern}} & \multicolumn{4}{c|}{\textbf{Random forest}} & \multicolumn{4}{c}{\textbf{J48 Decision Tree}}\\
		\cline{2-9}
		& \textbf{Cov} & \textbf{Pre} & \textbf{Rec} & \textbf{F1} & \textbf{Cov} & \textbf{Pre} & \textbf{Rec} & \textbf{F1} \\
		\toprule
		\textbf{*CF$\rightarrow$CF} & 83 & 71 & 72 & 71 & 69 & 60 & 63 & 61\\
		\textbf{*CF$\rightarrow$AF} & 82 & 75 & 78 & 76 & 67 & 62 & 69 & 65\\
		\textbf{*CF$\rightarrow$AV} & 81 & 74 & 78 & 76  & 60 & 63 & 67 & 64\\
		\bottomrule
		\multirow{2}{*}{\textbf{Pattern}} & \multicolumn{4}{c|}{\textbf{AdaBoost (default)}} & \multicolumn{4}{c}{\textbf{Naive Bayes}}\\
		\cline{2-9}
		& \textbf{C} & \textbf{P} & \textbf{R} & \textbf{F} & \textbf{C} & \textbf{P} & \textbf{R} & \textbf{F} \\
		\toprule
		\textbf{*CF$\rightarrow$CF} & 50 & 54 & 71 & 62 & 61 & 56 & 50 & 53\\
		\textbf{*CF$\rightarrow$AF} & 51 & 68 & 65 & 66 & 78 & 65 & 50 & 57\\
		\textbf{*CF$\rightarrow$AV} & 47 & 57 & 70 & 64 & 72 & 61 & 52 & 56\\
		\bottomrule
	\end{tabular}
	%}
	%\vspace{-1.5em}
	%\end{wraptable}
\end{table}


For Adaboost.M1, the default base classifier in Weka is Decision Stumps, we also applied Random Forest as the base classifier to do the prediction, as shown in Table~\ref{tab:1cf1c_adaboost}, ~\ref{tab:1af1c_adaboost}, and ~\ref{tab:1av1c_adaboost}.
\begin{table}
	\centering
	\scriptsize
	%\footnotesize
	%\vspace{-2em}
	\caption{Comparison results between \tool (AdaBoost + Random Forest) and ROSE
		for {*CF$\xrightarrow{f}$CF} tasks}
	%\vspace{1em}
	\label{tab:1cf1c_adaboost}
	%\resizebox{\columnwidth}{!}{%
	\begin{tabular}{C{1.2cm}|R{0.6cm} R{0.6cm} R{0.6cm} R{0.6cm} | R{0.6cm} R{0.6cm} R{0.6cm} R{0.6cm}}
		\toprule
		\multirow{2}{*}{\textbf{Project}} & \multicolumn{4}{c|}{\textbf{\tool}} & \multicolumn{4}{c}{\textbf{ROSE}}\\
		\cline{2-9}
		& \textbf{Cov} & \textbf{Pre} & \textbf{Rec} & \textbf{F1} & \textbf{Cov} & \textbf{Pre} & \textbf{Rec} & \textbf{F1} \\
		\toprule
		Node.js & 77 & 68 & 69 & 69 & 61 & 24 & 56& 34\\
		Meteor & 88 & 72 & 70 & 71 & 46 & 16 & 43 & 24\\
		Ghost & 73 & 67 & 74 & 71  & 50 & 20 & 53 & 29\\
		Habitica & 80 & 80 & 78 & 79 & 40 & 7 & 37 & 12\\
		PDF.js & 71 & 77 & 81 & 79 & 29 & 27 & 41 & 33\\
		React & 91 & 86 & 76 & 81 & 32 & 59 & 70 & 64\\
		Serverless & 84 & 77 & 79 & 78  & 64& 20 & 75 & 32\\
		Webpack & 89 & 71 & 81 & 75 & 50 & 7 & 29 & 12\\
		%Storybook & 66 & 100 & 100 & 100 & 0 & - & - & -\\
		%Electron & 100 & 92 & 94 & 93 & 63 & 20 & 83 & 34 \\
		\bottomrule
		\textbf{WA} & \textbf{83} & \textbf{72} & \textbf{73} & \textbf{73} & \textbf{53} & \textbf{21} & \textbf{52} & \textbf{29}\\
		\bottomrule
	\end{tabular}
	%}
	%\vspace{-1.5em}
	%\end{wraptable}
\end{table}


\begin{table}
	\centering
	\scriptsize
	%\footnotesize
	\vspace{1em}
	\caption{Comparison results between \tool (AdaBoost + Random Forest) and ROSE for {*CF$\xrightarrow{f}$AF} tasks}
	%\vspace{1em}
	\label{tab:1af1c_adaboost}
	%\resizebox{\columnwidth}{!}{%
	\begin{tabular}{C{1.2cm}|R{0.6cm} R{0.6cm} R{0.6cm} R{0.6cm} | R{0.6cm} R{0.6cm} R{0.6cm} R{0.6cm}}
		\toprule
		\multirow{2}{*}{\textbf{Project}} & \multicolumn{4}{c|}{\textbf{\tool}} & \multicolumn{4}{c}{\textbf{ROSE}}\\
		\cline{2-9}
		& \textbf{Cov} & \textbf{Pre} & \textbf{Rec} & \textbf{F1} & \textbf{Cov} & \textbf{Pre} & \textbf{Rec} & \textbf{F1} \\
		\toprule
		Node.js & 79 & 69 & 74 & 72 & 59 & 20 & 52 & 29\\
		Meteor & 86 & 77 & 82 & 80 & 40 & 22 & 44 & 29\\
		Ghost & 85 & 86 & 85 & 85  & 46 & 18 & 46 & 26\\
		Habitica & 87 & 77 & 85 & 81 & 56 & 4 & 23 & 7\\
		PDF.js & 65 & 87 & 88 & 87 & 22 & 9 & 28 & 14\\
		React & 71 & 84 & 82 & 83 & 16 & 66 & 7 & 13\\
		Serverless & 84 & 71 & 85 & 77  & 73& 19 & 59 & 29\\
		Webpack & 75 & 79 & 85 & 82 & 53 & 16 & 46 & 24\\
		\bottomrule
		\textbf{WA} & \textbf{81} & \textbf{76} & \textbf{80} & \textbf{78} & \textbf{54} & \textbf{21} & \textbf{48} & \textbf{28}\\
		\bottomrule
	\end{tabular}
	%}
	%\vspace{-1.5em}
	%\end{wraptable}
\end{table}



\begin{table}
	\centering
	\scriptsize
	%\footnotesize
	\vspace{1em}
	\caption{Comparison results between \tool (AdaBoost + Random Forest) and ROSE for {*CF$\xrightarrow{v}$AV} tasks}
	%\vspace{1em}
	\label{tab:1av1c_adaboost}
	%\resizebox{\columnwidth}{!}{%
	\begin{tabular}{C{1.2cm}|R{0.6cm} R{0.6cm} R{0.6cm} R{0.6cm} | R{0.6cm} R{0.6cm} R{0.6cm} R{0.6cm}}
		\toprule
		\multirow{2}{*}{\textbf{Project}} & \multicolumn{4}{c|}{\textbf{\tool}} & \multicolumn{4}{c}{\textbf{ROSE}}\\
		\cline{2-9}
		& \textbf{Cov} & \textbf{Pre} & \textbf{Rec} & \textbf{F1} & \textbf{Cov} & \textbf{Pre} & \textbf{Rec} & \textbf{F1} \\
		\toprule
		Node.js & 79 & 72 & 77 & 74 & 55 & 20 & 65 & 31\\
		Meteor & 72 & 77 & 84 & 81 & 26 & 2 & 14 & 4\\
		Ghost & 84 & 75 & 81 & 78  & 46 & 18 & 46 & 26\\
		Habitica & 89 & 82 & 85 & 83 & 27 & 20 & 45 & 28\\
		PDF.js & 78 & 87 & 84 & 85 & 20 & 4 & 28 & 8\\
		React & 89 & 73 & 78 & 76 & 36 & 8 & 33 & 13\\
		Serverless & 70 & 80 & 85 & 82  & 34 & 0 & 0 & -\\
		Webpack & 87 & 86 & 83 & 85 & 36 & 8 & 33 & 13\\
		\bottomrule
		\textbf{WA} & \textbf{79} & \textbf{76} & \textbf{81} & \textbf{78} & \textbf{45} & \textbf{17} & \textbf{54} & \textbf{25}\\
		\bottomrule
	\end{tabular}
	%}
	%\vspace{-1.5em}
	%\end{wraptable}
\end{table}
\end{comment} 
